Chemistry Along Accretion Streams in a Viscously-Evolving Protoplanetary Disk

The composition of a protoplanetary disk is set by a combination of interstellar inheritance and gas and grain surface chemical reactions within the disk. The survival of inherited molecules, as well as the disk in situ chemistry depends on the local temperature, density and irradiation environment, which can change over time due to stellar and disk evolution, as well as transport in the disk. We address one aspect of this coupling between the physical and chemical evolution in disks by following accretion streamlines of gas and small grains in the disk midplane, while simultaneously taking the evolving star into account. This approach is computationally efficient and enables us to take into account changing physical conditions without reducing the chemical network. We find that many species are enhanced in the inner disk midplane in the dynamic model due to inward transport of cosmic-ray driven chemical products, resulting in, e.g., orders-of magnitude hydrocarbon enhancements at 1 au, compared to a static disk. For several other chemical families, there is no difference between the static and dynamic models, indicative of a robust chemical reset, while yet others show differences between static and dynamic models that depend on complex interactions between physics and chemistry during the inward track. The importance of coupling dynamics and chemistry when modeling the chemical evolution of protoplanetary disks is thus depends on what chemistry is of interest.

==> tbl_results2_05au_fin_tot_.tex <==
C${}_{2}$H${}_{2}$ & $1.3 \times 10^{-9}$ & $4.8 \times 10^{1}$\\
C${}_{2}$H${}_{2}$N & $2.2 \times 10^{-10}$ & $3.2 \times 10^{2}$\\
C${}_{2}$H${}_{3}$N & $1.5 \times 10^{-10}$ & $2.1 \times 10^{2}$\\
C${}_{2}$H${}_{4}$ & $3.5 \times 10^{-9}$ & $9.6 \times 10^{1}$\\
C${}_{3}$ & $2.1 \times 10^{-10}$ & $2.2 \times 10^{1}$\\
C${}_{3}$H${}_{2}$ & $1.3 \times 10^{-10}$ & $2.2 \times 10^{3}$\\
C${}_{3}$H${}_{3}$ & $1.6 \times 10^{-10}$ & $5.8 \times 10^{4}$\\
C${}_{3}$H${}_{4}$ & $1.3 \times 10^{-10}$ & $1.0 \times 10^{3}$\\
CH${}_{3}$N & $1.9 \times 10^{-9}$ & $1.3 \times 10^{2}$\\
CH${}_{3}$OCH${}_{3}$ & $6.6 \times 10^{-8}$ & $6.0 \times 10^{1}$\\
CH${}_{5}$N & $1.2 \times 10^{-9}$ & $1.4 \times 10^{2}$\\
H${}_{2}$CO & $5.8 \times 10^{-8}$ & $2.2 \times 10^{4}$\\
HCOOCH${}_{3}$ & $3.1 \times 10^{-9}$ & $6.6 \times 10^{3}$\\
HNC & $1.1 \times 10^{-8}$ & $1.5 \times 10^{1}$\\
N${}_{2}$O & $8.5 \times 10^{-10}$ & $5.0 \times 10^{1}$\\
NH${}_{2}$CHO & $6.9 \times 10^{-8}$ & $2.8 \times 10^{1}$\\
NO & $6.1 \times 10^{-10}$ & $4.1 \times 10^{4}$

==> tbl_results2_05au_init_tot_.tex <==
HNC & $1.1 \times 10^{-8}$ & $8.1 \times 10^{1}$\\
NO & $6.1 \times 10^{-10}$ & $1.5 \times 10^{3}$

==> tbl_results2_10au_fin_tot.tex <==
NC${}_{4}$N & $2.5 \times 10^{-10}$ & $8.0 \times 10^{2}$

==> tbl_results2_10au_fin_tot_.tex <==
NC${}_{4}$N & $2.5 \times 10^{-10}$ & $8.0 \times 10^{2}$

==> tbl_results2_10au_init_tot.tex <==
C${}_{2}$H${}_{2}$N & $1.5 \times 10^{-9}$ & $2.0 \times 10^{1}$

==> tbl_results2_10au_init_tot_.tex <==
C${}_{2}$H${}_{2}$N & $1.5 \times 10^{-9}$ & $2.0 \times 10^{1}$
